Evidence for the Higgs-boson Yukawa coupling to tau leptons with the ATLAS detector

Results of a search for $H \to \tau \tau$ decays are presented, based on the full set of proton-proton collision data recorded by the ATLAS experiment at the LHC during 2011 and 2012. The data correspond to integrated luminosities of 4.5 $\rm{fb}^{-1}$ and 20.3 $\rm{fb}^{-1}$ at centre-of-mass energies of $\sqrt{s}$ = 7 TeV and $\sqrt{s}$ = 8 TeV respectively. All combinations of leptonic ($\tau \to \ell \nu \bar \nu$ with $\ell = e, \mu$) and hadronic ($\tau \to \rm{hadrons} \nu$) tau decays are considered. An excess of events over the expected background from other Standard Model processes is found with an observed (expected) significance of 4.5 (3.4) standard deviations. This excess provides evidence for the direct coupling of the recently discovered Higgs boson to fermions. The measured signal strength, normalised to the Standard Model expectation, of $\mu = 1.43 ^{+0.43}_{-0.37}$ is consistent with the predicted Yukawa coupling strength in the Standard Model.

==> Makefile <==
#export TEXINPUTS=.//:/usr/share/texmf/tex/latex//:../../../external//:

#-------------------------------------------------------------------------------
# user variables
#-------------------------------------------------------------------------------
doc = paper_main
bib = bibliography
latex = latex # latex or pdflatex
gv_scale = 1

#-------------------------------------------------------------------------------

deps := $(wildcard *.tex *.bib figs/*.pdf figs/*.eps)  $(bib).bbl
alltexs := $(wildcard *.tex)
texs = $(filter-out $(doc).tex,$(alltexs))
 
#-------------------------------------------------------------------------------
# targets
#-------------------------------------------------------------------------------
#default: $(doc).pdf show
default: $(doc).pdf
	@echo "--------------------------------------------------------------------------------"
	@echo "make $@"
	@echo "--------------------------------------------------------------------------------"
	@echo "Your dependencies are: $(deps)"

$(doc).pdf: $(deps)
	@echo "--------------------------------------------------------------------------------"
	@echo "make $@"
	@echo "--------------------------------------------------------------------------------"
	@make $(latex)

%.bbl: %.bib
	@echo "--------------------------------------------------------------------------------"
	@echo "make $@"
	@echo "--------------------------------------------------------------------------------"
	$(latex) $(doc).tex
	$(latex) $(doc).tex
	bibtex $(doc)
	$(latex) $(doc).tex
	$(latex) $(doc).tex

.PHONY: pdflatex
pdflatex:
	@echo "--------------------------------------------------------------------------------"
	@echo "make $@"
	@echo "--------------------------------------------------------------------------------"
	pdflatex $(doc).tex
	pdflatex $(doc).tex

.PHONY: latex
latex: $(doc).ps
	@echo "--------------------------------------------------------------------------------"
	@echo "make $@"
	@echo "--------------------------------------------------------------------------------"
	@if [[ "$(UNAME_S)" == "Darwin" ]]; then \
		pstopdf $(doc).ps; \
	else \
		ps2pdf -sPAPERSIZE=a4 $(doc).ps $(doc).pdf; \
	fi

$(doc).ps: $(doc).dvi
	@echo "--------------------------------------------------------------------------------"
	@echo "make $@"
	@echo "--------------------------------------------------------------------------------"
	dvips -o $(doc).ps $(doc).dvi

$(doc).dvi: $(doc).tex
	@echo "--------------------------------------------------------------------------------"
	@echo "make $@"
	@echo "--------------------------------------------------------------------------------"
	latex $(doc).tex
	latex $(doc).tex

.PHONY: over
over: realclean default
	@echo "--------------------------------------------------------------------------------"
	@echo "make $@"
	@echo "--------------------------------------------------------------------------------"

.PHONY: clean
clean:
	@echo "--------------------------------------------------------------------------------"
	@echo "make $@"
	@echo "--------------------------------------------------------------------------------"
	rm -f *.aux $(doc).bbl $(doc).blg $(doc).dvi $(doc).log $(doc).nav $(doc).out $(doc).ps $(doc).pdf $(doc).snm $(doc).toc *~

.PHONY: realclean
realclean: clean
	@echo "--------------------------------------------------------------------------------"
	@echo "make $@"
	@echo "--------------------------------------------------------------------------------"
	rm -f $(doc).pdf

.PHONY: show
show:
	@echo "--------------------------------------------------------------------------------"
	@echo "make $@"
	@echo "--------------------------------------------------------------------------------"
	@if [ `ps ax | grep -v grep | grep gv | grep -c $(doc).pdf` -eq 0 ]; then\
		echo "Opening document with ghostview...";\
		sleep 2;\
		gv -antialias -watch -scale=$(gv_scale) -resize $(doc).pdf & \
	else \
		echo "Document is already open with ghostview.";\
	fi


